Tracking State Changes in Procedural Text: A Challenge Dataset and Models for Process Paragraph Comprehension

We present a new dataset and models for comprehending paragraphs about processes (e.g., photosynthesis), an important genre of text describing a dynamic world. The new dataset, ProPara, is the first to contain natural (rather than machine-generated) text about a changing world along with a full annotation of entity states (location and existence) during those changes (81k datapoints). The end-task, tracking the location and existence of entities through the text, is challenging because the causal effects of actions are often implicit and need to be inferred. We find that previous models that have worked well on synthetic data achieve only mediocre performance on ProPara, and introduce two new neural models that exploit alternative mechanisms for state prediction, in particular using LSTM input encoding and span prediction. The new models improve accuracy by up to 19%. The dataset and models are available to the community at http://data.allenai.org/propara.

==> problem-description1.tex <==
\section{Problem Description}

%\subsection{Motivation}

Our dataset, \emph{ProPara}, focuses on a particular genre of procedural text, namely
simple scientific processes (e.g., photosynthesis, erosion).  In addition,
we aim to test a system's understanding of the process description through question answering.

A system that understands a process paragraph should be able
to answer questions such as: ``\textit{What are the inputs to the process?}'', 
``\textit{What is converted into what?}'', ``\textit{Where does the conversion take place?}''
and ``\textit{Where is X transported from/to?}''\footnote{For example, science exams 
pose such questions to test student's understanding of the text in various ways.}
%
Many of these questions reduce to understanding the
basic dynamics of entities in the process:
\begin{enu}
\item[1.] {\bf What} is created/destroyed/moved?
\item[2.] {\bf When} are those created/destroyed/moved?
\item[3.] {\bf Where} are those created/destroyed/moved?
\end{enu}
For example, the inputs of the process are the consumed/destroyed items; the 
outputs are the created items; etc. Thus, if we can track entities' existence
and location across the process, we can answer these higher level questions.
Following this design, we describe the details of the \emph{state} representation of processes in \emph{ProPara}
and the QA task.

\paragraph{Process State Representation}
The states of the world throughout the whole process are represented as a grid.  Each column denotes 
a \emph{participant} entity (a span in the paragraph, typically a noun phrase) that undergoes some 
creation, destruction, or movement in the process.  Each row denotes the \emph{states} of all the 
participants after a \emph{step}.  We view each sentence as a step that may change the state of one or more participants.
Therefore, a process paragraph with $m$ sentences and $n$ participants will result in an $(m+1) \times n$ 
grid representation. Each cell $l_{ij}$ in this grid records the \emph{location} of the $j$-th participant
after the $i$-th step, and $l_{0j}$ stores the location of $j$-th participant before the process.\footnote{We only trace 
locations in this work, but the representation can be easily extended to store other properties (e.g., temperature) 
of the participants.}  Figure~\ref{participant-grid} shows one example of this representation.



\paragraph{Question Answering Task} \label{sect:end_task}

To evaluate the understanding of a process paragraph, a system is asked to answer 10 questions grouped in 3 categories.
Given a process paragraph and a participant entity $e$ in it, identify:

\noindent
(1) {\bf Is} $e$ created (destroyed, moved) in the process?

\noindent
(2) {\bf When} (step \#) is $e$ created (destroyed, moved)?

\noindent
(3) {\bf Where} is $e$ created (destroyed, moved from/to)?

These questions measure the system's ability to track locational state changes:
a creation is a change from ``not exists" to a location; a destruction is a change from a location to ``not exists";
and a move is a change from one location to another. 

